Classification via Two-Way Comparisons

Given a weighted, ordered query set $Q$ and a partition of $Q$ into classes, we study the problem of computing a minimum-cost decision tree that, given any query $q$ in $Q$, uses equality tests and less-than comparisons to determine the class to which $q$ belongs. Such a tree can be much smaller than a lookup table, and much faster and smaller than a conventional search tree. We give the first polynomial-time algorithm for the problem. The algorithm extends naturally to the setting where each query has multiple allowed classes.

==> FIGURES/TREES/inversion.tex <==
\newcommand{\KA}{4}
\newcommand{\KB}{3}
\newcommand{\KC}{2}
\newcommand{\KD}{1}
\newcommand{\SETSEP}{\cup}
\newcommand{\WTSEP}{\,\,+\,\,}

\bracketset{action character=@}
\centering
\noindent
\A
\adjustbox{valign=t,scale = 0.82}{
  \begin{generictree}
    [{$=\KA$},
      [{$\KA$}, weight={$\mathbf 4$}]
      [{$=\KB$}, s sep=1.4em,
        [{$\KB$}, weight={$\mathbf 4$}]
        [{$=\KD$},
          [{$\KD$}, weight={$0$}]
          % [{$(-\infty, \infty) \setminus \{\KD,\KB,\KA\}$},
          [{$\iota_1 \SETSEP \iota_2 \SETSEP \{\KC\} \SETSEP \iota_3\SETSEP \iota_4\SETSEP \iota_\infty$},
            % weight={$0{,}\, 0{,}\, 0{,}\, \mathbf 5{,}\, 2{,}\, 1$}
            weight={$
                  1
                  \WTSEP
                  2
                  \WTSEP
                  \mathbf 5
                  \WTSEP
                  0
                  \WTSEP
                  0
                  \WTSEP
                  0
                $}]
        ]
      ]
    ]
  \end{generictree}
}
\hspace*{-2em}
\B
\adjustbox{valign=t,scale = 0.82}{
  \begin{generictree}
    [{$=\KC$},
      [{$\KC$},  weight={$5$}]
      [{$=\KA$},
        [{$\KA$},  weight={$4$}]
        [{$=\KB$},
          [{$\KB$},  weight={$4$}]
          [{$=\KD$},
            [{$\KD$},  weight={$0$}]
            % [{$(-\infty, \infty) \setminus \{\KD,\KC,\KB, \KA\}$},
            [{$\iota_1 \SETSEP \iota_2 \SETSEP \iota_3\SETSEP \iota_4\SETSEP \iota_\infty$},
              %weight={$0\WTSEP 0\WTSEP 0\WTSEP 2\WTSEP 1$}]
              weight={$1\WTSEP 2\WTSEP 0\WTSEP 0\WTSEP 0$}]
          ]
        ]
      ]
    ]
  \end{generictree}
}
\hspace*{-3em}
\C
\adjustbox{valign=t,scale = 0.82}{
  \begin{generictree}
    [{$< \KB$},
      [{$=\KC$},
        [{$\KC$},  weight={$5$}]
        [{$=\KD$},
          [{$\KD$},  weight={$0$}]
          % [{$(-\infty, \KB)\setminus \{\KD, \KC\}$},
          [{$\iota_1 \SETSEP \iota_2 \SETSEP\iota_3$},
            weight={$1\WTSEP 2\WTSEP 0$}]
        ]
      ]
      [{$=\KA$},
        [{$\KA$},  weight={$4$}]
        [{$=\KB$},
          [{$\KB$},  weight={$4$}]
          % [{$(\KB, \infty)\setminus \{\KA\}$},
          [{$\iota_4\SETSEP \iota_\infty$},
            weight={$0\WTSEP 0$}]
        ]
      ]
    ]
  \end{generictree}
}
\hspace*{-2em}
\D
\hspace*{0.2em}
\adjustbox{valign=t,scale = 0.82,raise=10pt}{
  \(
  \begin{array}{| c @{\,} c @{} c @{} |}
    \multicolumn{1}{ c }{\text{query}} & \text{cls} & \multicolumn{1}{ r @{} }{\text{wt}} \\ \hline
    (-\infty,\KD)                      & \text z    & 1                                   \\
    ~\KD                               & \text A    & 0                                   \\
    (\KD,\KC)                          & \text z    & 2                                   \\
    ~\KC                               & \text z    & 5                                   \\
    (\KC,\KB)                          & \text z    & 0                                   \\
    ~\KB                               & \text B    & 4                                   \\
    (\KB, \KA)                         & \text z    & 0                                   \\
    ~\KA                               & \text C    & 4                                   \\
    (\KA,\infty)                       & \text z    & 0                                   \\
    \hline
  \end{array}
  \)
}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "00_main"
%%% End:


==> FIGURES/TREES/lead-example.tex <==

\centering
\noindent
\A \hspace*{-2em}
\adjustbox{valign=t, scale=0.8}{
  \begin{generictree}
    [{$= 15$}, s sep=2em,
      [{15}, weight={H}]
      [{$< 26$},
        [{$< 18$},
          [{$< 11$},
            [{$< 7$},
              [{$< 5$},
                [{$= 3$},
                  [{3}, weight={C}]
                  [{$= 2$},
                    [{2}, weight={B}]
                    [{1{,} 4}, weight={A}]
                  ]
                ]
                [{$< 6$},
                  [{5}, weight={D}]
                  [{6}, weight={B}]
                ]
              ]
              [{$< 9$},
                [{$< 8$},
                  [{7}, weight={E}]
                  [{8}, weight={F}]
                ]
                [{$< 10$},
                  [{9}, weight={A}]
                  [{10}, weight={G}]
                ]
              ]
            ]
            [{11-14{,} 16-17}, weight={H}]
          ]
          [{$< 22$},
            [{18-21}, weight={I}]
            [{22-25}, weight={H}]
          ]
        ]
        [{$< 42$},
          [{26-41}, weight={J}]
          [{42-50}, weight={K}]
        ]
      ]
    ]
  \end{generictree}
}
\hspace*{0.7em}
\B
\hspace*{0.7em}
\adjustbox{valign=t, scale=0.82, raise=10pt}{
  \begin{tabular}{|rc@{}r|}
    \multicolumn{1}{r}{$q$} & cls & \multicolumn{1}{r@{\,}}{wt} \\ \hline
    \rule{0pt}{1em}
    1                       & A   & 6                           \\
    2                       & B   & 7                           \\
    3                       & C   & 7                           \\
    4                       & A   & 6                           \\
    5                       & D   & 8                           \\
    6                       & B   & 8                           \\
    7                       & E   & 7                           \\
    8                       & F   & 6                           \\
    9                       & A   & 8                           \\
    10                      & G   & 7                           \\
    11                      & H   & 10                          \\
    12                      & H   & 11                          \\
    13                      & H   & 10                          \\
    14                      & H   & 9                           \\
    15                      & H   & 500                         \\
    16                      & H   & 9                           \\
    17                      & H   & 10                          \\
    \hline
  \end{tabular}\hspace*{-3pt}
  \begin{tabular}{rc@{}r|}
    \multicolumn{1}{c}{$q$} & cls & \multicolumn{1}{r}{wt} \\ \hline
    \rule{0pt}{1em}
    18                      & I   & 10                     \\
    19                      & I   & 8                      \\
    20                      & I   & 15                     \\
    21                      & I   & 17                     \\
    22                      & H   & 7                      \\
    23                      & H   & 8                      \\
    24                      & H   & 15                     \\
    25                      & H   & 10                     \\
    26                      & J   & 1                      \\
    27                      & J   & 2                      \\
    28                      & J   & 2                      \\
    29                      & J   & 1                      \\
    30                      & J   & 2                      \\
    31                      & J   & 2                      \\
    32                      & J   & 100                    \\
    33                      & J   & 1                      \\
    34                      & J   & 2                      \\
    \hline
  \end{tabular}\hspace*{-3pt}
  \begin{tabular}{rc@{}c@{}|}
    \multicolumn{1}{c}{$q$} & cls & \multicolumn{1}{c}{wt} \\ \hline
    \rule{0pt}{1em}
    35                      & J   & 2                      \\
    36                      & J   & 2                      \\
    37                      & J   & 1                      \\
    38                      & J   & 1                      \\
    39                      & J   & 1                      \\
    40                      & J   & 2                      \\
    41                      & J   & 1                      \\
    42                      & K   & 3                      \\
    43                      & K   & 3                      \\
    44                      & K   & 3                      \\
    45                      & K   & 3                      \\
    46                      & K   & 3                      \\
    47                      & K   & 3                      \\
    48                      & K   & 3                      \\
    49                      & K   & 3                      \\
    50                      & K   & 3                      \\
                            &     &                        \\
    \hline
    % \multicolumn{1}{r}{~} &  & \multicolumn{1}{l}{~}\\
  \end{tabular}
}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "00_main"
%%% End:


==> FIGURES/TREES/other_rotations.tex <==
\bracketset{action character=@}

\adjustbox{scale=0.9, trim=20pt 0pt 0pt 0pt}{
  %  \newcommand{\X}{$\uA$}
  %  \newcommand{\Z}{$\uB$}
  %  \newcommand{\tA}{$\uC$}
  %  \newcommand{\tB}{$\uC'$}
  %  \newcommand{\tC}{$\uB'$}
  \newcommand{\X}{$a$}
  \newcommand{\Z}{$b$}
  \newcommand{\tA}{$c$}
  \newcommand{\tB}{$c'$}
  \newcommand{\tC}{$b'$}
  %  \newcommand{\rootTip}{Circle[open]}
  %  \newcommand{\brokenEdge}{edge label={node[midway,fill=white,yshift=0pt, inner ysep=2pt]{~}}}

  \begin{generictrees}
    [, phantom, for tree={l=0.3ex, s sep=1em}, s sep=1.5em,
      %    [, phantom, [{\large \A}, nodraw]]
      %    [, phantom,
      %    [{\X},
      %    [{\Z}, bright, edge={<-}
      %    [{\tA}, subtree]
      %    [{\tB}, subtree, bright, squigglyedge]
      %    ]
      %    [{\tC}, subtree, ]
      %    ]
      %    ]
      %    [, phantom, [, phantom, [{\large $\Rightarrow$ }, nodraw]]]
      %    [, phantom,
      %    [{\Z}, bright,
      %    [{\X},
      %    [{\tA}, subtree]
      %    [{\tC}, subtree,]
      %    ]
      %    [{\tB}, subtree, bright, ]
      %    ]
      %    ]
      %    [, phantom]
      %    [, phantom, [, phantom, l sep=-0.5em, [{\large or}, nodraw]]]
      %    [, phantom, [{\large \B}, nodraw]]
      [, phantom,
        [{\X},
          [{\Z}, bright, edge={<-}
            [{\tB}, subtree, bright,]
            [{\tA}, subtree]
          ]
          [{\tC}, subtree]
        ]
      ]
      [, phantom, [, phantom, [{\large $\Longrightarrow$ }, nodraw]]]
      [, phantom,
        [{\Z}, bright,
          [{\tB}, subtree, bright]
          [{\X},
            [{\tA}, subtree]
            [{\tC}, subtree]
          ]
        ]
      ]
    ]
  \end{generictrees}
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "00_main"
%%% End:
%
%\bracketset{action character=@}
%
%\adjustbox{scale=0.9, trim=20pt 0pt 0pt 0pt}{
%  \newcommand{\X}{$\uA$}
%  \newcommand{\Z}{$\uB$}
%  \newcommand{\tA}{$\uC$}
%  \newcommand{\tB}{$\uC'$}
%  \newcommand{\tC}{$\uB'$}
%  \newcommand{\rootTip}{Circle[open]}
%  \begin{generictrees}
%    [, phantom, for tree={l=0.3ex, s sep=1em}, s sep=1.8em,
%    [, % interior,
%    [{\X}, edge={{\rootTip}-},
%    [{\Z}, edge={-},
%    [{\tA}, subtree]
%    [{\tB}, brighttree, squigglyedge]
%    ]
%    [{\tC}, brighttree, squigglyedge]
%    ]
%    ]
%    [, phantom, [{\large\ \hspace{0in} $\Longrightarrow$ \hspace*{-0.1in}\ }, nodraw]]
%    [, s sep=0.5em, l=0em, xshift=2pt, yshift=-1pt,
%    [, xshift=0em, l sep=-0.5em, edge={draw=none}, nodraw,
%    [, xshift=0em, edge={draw=none}, nodraw,
%    [{\tA}, subtree, edge={draw=none}, xshift=-1em,]
%    ]
%    ]
%    [, l sep=-0.5em, nodraw, xshift=0em, edge={{\rootTip}-},
%    [{\Z}, edge={draw=none}, xshift=0em,
%    [, nodraw]
%    [{\tB}, brighttree, squigglyedge]
%    ]
%    [, nodraw, edge={draw=none}]
%    ]
%    [, xshift=0em, l sep=-0.5em, edge={draw=none}, nodraw,
%    [{\X}, edge={draw=none}, xshift=0em,
%    [, nodraw]
%    [{\tC}, brighttree, squigglyedge]
%    ]
%    ]
%    ]
%    [, phantom, [{\large\ \hspace*{-0.1in} $\Longrightarrow$ \hspace{0.1in}\ }, nodraw]]
%    [,
%    [{\Z}, l=-10pt, edge={{\rootTip}-},
%    [{\X}, edge={-},
%    [{\tA}, subtree]
%    [{\tC}, brighttree, squigglyedge]
%    ]
%    [{\tB}, brighttree, squigglyedge]
%    ]
%    ]
%    ]
%  \end{generictrees}
%}


==> FIGURES/TREES/three-way-vs-two-way.tex <==
\newcommand{\CMP}{{}\mathrel{?}}
\centering
\noindent
\A%\hspace*{-2em}
\adjustbox{valign=t,scale = 0.87}{
  \begin{ThreeWayTree}
    %
    [{$ \CMP 3$}, s sep=3.2em,
      [{$ \CMP 1$}, s sep=1.8em,
        [{$(-\infty, 1)$}, weight={15}]
        [1, calign with current, weight={8}]
        [{$ \CMP 2$}
          [{$(1, 2)$}, weight={21}]
          [2, calign with current, weight={2}]
          [{$(2, 3)$}, weight={8}]
        ]
      ]
      [3, calign with current, weight={8}]
      [{$ \CMP 4$}
        [{$(3, 4)$}, weight={4}]
        [4, calign with current, weight={33}]
        [{$(4,\infty)$}, weight={1}]
      ]
    ]
  \end{ThreeWayTree}
}
\hspace*{0.7em}
\B%\hspace*{-2em}
\adjustbox{valign=t,scale = 0.87}{
  \begin{generictree}
    %
    [{$<2$}
      [{$<1$}
        [{$(-\infty, 1)$}, weight={15}]
        [{$=1$},
          [1, weight={8}]
          [{$(1, 2)$}, weight={21}]
        ]
      ]
      [{$=4$}, s sep=1.8em,
        [4, weight={33}]
        [{$<3$}
          [{$=2$},
            [2, weight={2}]
            [{$(2, 3)$}, weight={8}]
          ]
          [{$=3$},
            [3, weight={8}]
            [{$<4$},
              [{$(3, 4)$}, weight={4}]
              [{$(4,\infty)$}, weight={1}]
            ]
          ]
        ]
      ]
    ]
  \end{generictree}
}
% \hspace*{-1em}
% \C
% % \hspace*{0.7em}
% \adjustbox{valign=t,scale = 0.9, raise=10pt}{
%   \(
%   \begin{array}{| l @{\,} r |}
%     \multicolumn{1}{ l }{~q} & \multicolumn{1}{ r }{\text{wt}}\\ \hline
%     (-\infty, 1) & 15\\
%     ~1 & 8\\
%     (1, 2) & 21\\
%     ~2 & 2\\
%     (2,3) & 8\\
%     ~3 & 8\\
%     (3,4) & 4 \\
%      ~4 & 33\\
%     (4, \infty) & 1\\ \hline
%   \end{array}
%   \)
% }

